Disk Harmonics for Analysing Curved and Flat Self-affine Rough Surfaces and the Topological Reconstruction of Open Surfaces

When two bodies get into contact, only a small portion of the apparent area is actually involved in producing contact and friction forces, because of the surface roughnesses. It is therefore crucial to accurately describe the morphology of rough surfaces for instance by extracting the fractal dimension and the so-called Hurst exponent which is a typical signature of rough surfaces. This can be done using harmonic decomposition, which is easy for periodic and nominally flat surfaces since Fourier transforms allow fast and reliable decomposition. Yet, it remains a challenging task in the general curved and non-periodic cases, where more appropriate basis functions must be used. In this work, disk harmonics based on Fourier-Bessel basis functions are employed for decomposing open single-edge genus-0 surfaces (no holes) as a practical and fast alternative to characterise self-affine rough surfaces with the power Fourier-Bessel spectral density. An analytical relationship between the power spectrum density decay and the Hurst exponent is derived through an extension of the Wiener-Khinchin theorem, in the special case where surfaces are assumed self-affine and isotropic. Finally, this approach is demonstrated to successfully measure the fractal dimension, and the Hurst exponent, without introducing typical biases coming from basis functions boundary conditions, surface discretisation or curvature of the surface patches. This work opens the path for contact mechanics studies based on the Fourier-Bessel spectral representation of curved and rough surface morphologies. All implementation details for this method are available under GNU LGPLv3 terms and conditions.

==> app_A_real_basis.tex <==
\par
As real numbers require half the computer memory to preserve as complex ones, real harmonics expression could be useful for expanding signals with ultra-high degrees. Similar to the real spherical harmonics derived in Blanco et al. (1997) \cite{Blanco1997} and Ritchie et al. (1999) \cite{REF:8}, we can find an equivalent real expression for our disk harmonics basis $D_m^k (\rho, \phi)$ in Eq.~(\ref{EQN:FOUR_BESS_final}). To form this equivalency, we start by assuming that the basis functions corresponding to $m>0$ will be represented by cosine terms and those with $m<0$ will be expressed by sines. By exploiting Euler's formula on the angular part of the basis, Eq.~(\ref{EQN:LAP_FOURIER}) can be adapted as such:
\begin{equation*}
    \cos (m \phi) = \frac{\Phi_m (\phi) + \Phi_m^{*} (\phi)}{2} = \frac{e^{i m \phi} + e^{-i m \phi}}{2},
\end{equation*}
\begin{equation*}
    \sin (m \phi) = \frac{\Phi_m (\phi) - \Phi_m^{*} (\phi)}{2} = \frac{e^{i m \phi} - e^{-i m \phi}}{2i}.
\end{equation*}
Then the normalisation factor for the angular portion can be computed such that: 
\begin{equation}
    \int_0^{2 \pi} \cos (m \phi) \cos (m' \phi)  d \phi = \pi \delta_{mm^{\prime}}.
    \label{EQN:REAL_NORM_FOURIER}
\end{equation}
Similarly,
\begin{equation}
\int_0^{2 \pi} \sin (m \phi) \sin (m' \phi)  d \phi = \pi \delta_{mm^{\prime}}.
\end{equation}
Comparison with Eq.~(\ref{EQN:LAP_FOURIER}) shows that there will be a change of factor $\sqrt{2}$ in the final normalisation. Thus, the new orthonormal real Fourier-Bessel basis functions $\tilde{D}_m^k (\rho, \phi)$ can be written as:
\begin{equation}
\tilde{D}_m^k (\rho, \phi) = 
\left\{
\begin{array}{ll}
      \sqrt{2} N_m^k J_m\big( l(m)_k~\rho \big) \cos(m\phi)& m >0\\
      N_m^k J_m\big( l(m)_k~\rho \big)& m = 0\\
      \sqrt{2} N_{|m|}^k J_{|m|}\big( l(|m|)_k~\rho \big) \sin(|m|\phi)& m < 0\\
\end{array}
\right..
\label{EQN:REAL_FOUR_BESS_final}
\end{equation}
\par
Although the latter expression implies rotation about the $z$-axis from the original complex basis, the computed PSD should always remain invariant to the rotations of the basis functions or signals.

==> app_B_PSD_results.tex <==
% \par
% The curvature results shown in Figure \ref{FIG:MORE_CURV_PSD_VS_NORM} demonstrate the normalisation for the curvature of the spherical caps and the resulting distortion on the caps for large $R_{\theta_c}$. As can be seen in Figure \ref{FIG:MORE_CURV_PSD_VS_NORM}(A) for small curvatures where $R_{\theta_c} \leq 1$, the distortion is very low and the PSDs almost all match. However, for larger values, the projection distortion degenerates, so the PSD decay rate deviates from the real expected value.

% \begin{figure*}
% \centering
% \includegraphics[width=0.9\textwidth]{Figures/curv_norm_H_0.8.pdf}%
% \caption{Effects of curvature for rough spherical patches with various radii $R_{\theta_c}$. A) Surface originally generated with $H=0.8$ and a seed number of $51$ with $R_{\theta_{c}} \in \{0.25, 0.5, 1, 1.5, 2, 3\}$. The fitted PSD here considers $2\leq k \leq 70$. The fitted decay slopes here were $\{-3.103, -3.159, -3.149, -3.208, -3.257, -3.316, -3.362\}$ for $R_{\theta_c} = 0.25, 0.5, \dots, 3$, respectively, considering that the analytical slope for $H=0.8$ is $-3.1$. B) The fitting slope for the generated surfaces after changing the starting fitting eigenvalue.
% \label{FIG:MORE_CURV_PSD_VS_NORM}
% }
% \end{figure*}

==> future.tex <==
\par
Many applications can be used with the herein proposed decomposition approach, and we are interested in expanding these methods in many different directions from what was proposed in this context, such as:
\begin{itemize}
    \item Adding a new application to harmonic decomposition methods by studying the shape-morphing structures, such as in \cite{Chen2018, vanRees2018}.
    
    \item Studying the roughness of real scanned surfaces, taking particular advantage of this method's scalability for constructing the PSD over several decades. This tool will be especially helpful in the experimental domain due to its ability to be invariant for the curvature of surfaces, as most natural surfaces have some embedded curvature.

    \item Studying the contacts of rough surfaces with various imposed curvatures.

    \item Generating rough self-affine surface patches with nonperiodic boundary conditions and with imposed curvature, which is relevant for many applications.
\end{itemize}
